ERNIE-SPARSE: Learning Hierarchical Efficient Transformer Through Regularized Self-Attention

Sparse Transformer has recently attracted a lot of attention since the ability for reducing the quadratic dependency on the sequence length. We argue that two factors, information bottleneck sensitivity and inconsistency between different attention topologies, could affect the performance of the Sparse Transformer. This paper proposes a well-designed model named ERNIE-Sparse. It consists of two distinctive parts: (i) Hierarchical Sparse Transformer (HST) to sequentially unify local and global information. (ii) Self-Attention Regularization (SAR) method, a novel regularization designed to minimize the distance for transformers with different attention topologies. To evaluate the effectiveness of ERNIE-Sparse, we perform extensive evaluations. Firstly, we perform experiments on a multi-modal long sequence modeling task benchmark, Long Range Arena (LRA). Experimental results demonstrate that ERNIE-Sparse significantly outperforms a variety of strong baseline methods including the dense attention and other efficient sparse attention methods and achieves improvements by 2.77% (57.78% vs. 55.01%). Secondly, to further show the effectiveness of our method, we pretrain ERNIE-Sparse and verified it on 3 text classification and 2 QA downstream tasks, achieve improvements on classification benchmark by 0.83% (92.46% vs. 91.63%), on QA benchmark by 3.24% (74.67% vs. 71.43%). Experimental results continue to demonstrate its superior performance.

==> algo/hst.tex <==
\begin{algorithm}[H]
\caption{HST: Hierarchical Sparse Transformer}
\label{algo:hst}
%\SetAlgoLined
 \begin{algorithmic}[1]
    \INPUT $T=t_i, i\in{[1, S]}$.
    
    % \State {$\bm{K_c} = \bm{H}\bm{W_{k,c}}$, $\bm{Q_c} = \bm{H}\bm{W_{q,c}}$, $\bm{V_c} = \bm{H}\bm{W_{v,c}}$,   $\bm{K_r} = \bm{P}\bm{W_{k,r}}$, $\bm{Q_r} = \bm{P}\bm{W_{q,r}}$}
    % \State {$\bm{A_{c\rightarrow c}} = \bm{Q_c K_c^{\intercal}}$} 
    % \For{$i=0,...,N-1$} 
    %     \State {$\bm{\tilde{A}_{c\rightarrow p}}[i,:] = \bm{Q_{c}}[i,:] \bm{K_r^{\intercal}}$} 
    % \EndFor
    \State {$\mathcal(R)=Representative Token id$}
    \State {$T'=\Phi(T) \in \mathrm{R}^{S \bmod B \times B}$}
    \State {$T''=[R, T'] \in  \mathrm{R}^{S \bmod B \times (B+1)}$}
    % \State {$\textbf{H_o} = \text{softmax}(\frac{\bm{\tilde{A}}}{\sqrt{3d}})\textbf{V_c}$}
   \OUTPUT ${H_o}$
 \end{algorithmic}

\end{algorithm}


==> fig/performance.tex <==


\begin{figure}[ht]
\centering
\begin{subfigure}[t]{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth]{attachments/SpeedTest.pdf}
    \label{perf_speed}
\end{subfigure}
~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
  %(or a blank line to force the subfigure onto a new line)
\begin{subfigure}[t]{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth]{attachments/MemoryTest.pdf}
    \label{perf_mem}
\end{subfigure}

\caption{Runtime and memory of full self-attention, \mname and BigBird \citep{zaheer2020bigbird}.}\label{fig:perf_mem_speed}
\vspace{-5mm}
\end{figure}


==> fig/problem_demo.tex <==


\begin{figure}[ht]
\centering
\begin{subfigure}[t]{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth]{./attachments/demo-1-1.pdf}
    \caption{Bottleneck in vanilla global sparse attention pattern}
    \label{bottleneck_problem_a}
\end{subfigure}
~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
  %(or a blank line to force the subfigure onto a new line)
\begin{subfigure}[t]{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth]{./attachments/demo-1-2.pdf}
    \caption{Our HST attention pattern}
    \label{bottleneck_problem_b}
\end{subfigure}
~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
%(or a blank line to force the subfigure onto a new line)
\begin{subfigure}[t]{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth]{./attachments/demo-2-1.pdf}
    \caption{Local information is the opposite of whole}
    \label{bottleneck_problem_c}
\end{subfigure}
~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
%(or a blank line to force the subfigure onto a new line)
\begin{subfigure}[t]{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth]{./attachments/demo-2-2.pdf}
    \caption{Our SOAR constraints output of different patterns}
    \label{bottleneck_problem_d}
\end{subfigure}

\caption{An illustration of problems with the Sparse Transformer mechanism, and our proposed methods of \mname. (a) shows global attention in Sparse Transformer causes bottleneck problems, and (b) shows \mname HST solution to the bottleneck problem. (c) shows the risk for semantic understanding of when split sentence into chunks. (d) shows the \mname model using different attention patterns to enhance model robustness.}\label{fig:bottleneck_problem}
\vspace{-5mm}
\end{figure}

% \begin{figure}[!ht]
%   \centering
%   \subfloat[][]{\includegraphics[width=.4\textwidth]{example-image-c}}\quad
%   \subfloat[][]{\includegraphics[width=.4\textwidth]{example-image-c}}\\
%   \subfloat[][]{\includegraphics[width=.4\textwidth]{example-image-c}}\quad
%   \subfloat[][]{\includegraphics[width=.4\textwidth]{example-image-c}}
%   \caption{First group of subfigures.}
%   \label{fig:sub1}
% \end{figure}

==> fig/soar_vs_rdrop.tex <==
\begin{figure}[]
\centering
\includegraphics[width=\linewidth]{attachments/soar_vs_rdrop.png}
%\vspace{-1cm}
\caption{effect of SOAR V.S. R-DROP}
\label{fig:svsr}
%\vspace{-0.5cm}
\end{figure}


==> table/adv.tex <==


\begin{table*}[ht]

\begin{subtable}{1\textwidth}
\centering
\small
  \begin{tabularx}{.85\linewidth}{
  >{\hsize=\hsize}X% 10% of 4\hsize
  >{\hsize=0.3\hsize}c% 30% of 4\hsize
  >{\hsize=0.4\hsize}c% 10% of 4\hsize
  >{\hsize=0.6\hsize}c% 30% of 4\hsize
  >{\hsize=0.4\hsize}c% 10% of 4\hsize
  >{\hsize=0.6\hsize}c% 30% of 4\hsize
  >{\hsize=0.4\hsize}c% 10% of 4\hsize
  >{\hsize=0.6\hsize}c% 30% of 4\hsize
 }
  \toprule \toprule
    \textbf{Models} &  \textbf{ListOps}  & \textbf{ListOps Adv} & \textbf{Text}   & \textbf{Text Adv} &  \textbf{Retrieval} & \textbf{Retrieval Adv} \\
\midrule 
    \mname          & \textbf{37.40}     & \textbf{18.90}       & \textbf{63.14}  & \textbf{63.17}    & \textbf{61.89}     & \textbf{61.80}     \\
     w/o SAR        &  37.30             & 9.65                 & 62.54           & 62.41             & 61.84              & 61.52              \\
  \end{tabularx}
\end{subtable}

\begin{subtable}{1\textwidth}
\centering
\small
  \begin{tabularx}{.85\linewidth}{
  >{\hsize=0.8\hsize}X
  >{\hsize=0.4\hsize}X
  >{\hsize=0.4\hsize}X
  >{\hsize=0.5\hsize}X
  >{\hsize=0.5\hsize}X
  }
 \hline
    \textbf{Models} & \textbf{Image} & {\textbf{Image Adv}} &  {\textbf{Pathfinder}}   & {\textbf{Pathfinder Adv}}   \\
\midrule 
    \mname          & \textbf{44.82} & {\textbf{42.78}}     &  {\textbf{78.22}}        & {\textbf{67.29}}             \\
     w/o SAR        & 43.59          & {40.12}              &  {76.39}                 & {51.00}                      \\
\bottomrule    \bottomrule
  \end{tabularx}
\end{subtable}
\caption{Performance of w/ and w/o \textbf{SAR}: We construct an adversarial dataset by shifting word to test the robustness of \mname and the sensitivity for sparse pattern shift.}
\label{adv}

\end{table*}




==> table/albation_saor.tex <==

\begin{table*}[]
%\tabcolsep 0.03in
    \centering
    \small
\begin{center}
% \resizebox{0.45\textwidth}{!}
% {
\begin{tabular}{l|ccccc|c}
  \hline \hline
    Models & Image & Pathfinder \\ 
\hline
    \mname & 45.28 & 78.77 \\
    w/o roll tokens & 43.48 & 77.96 (3/5 times) \\
\hline \hline
\end{tabular}
% } % small
\end{center}
\caption{Effective of rolling-tokens of \mname, }
\label{abl_saor}
\end{table*}



==> table/complexity_analysis.tex <==
\begin{table}[ht]
%\tabcolsep 0.03in
\small
\begin{center}
% \resizebox{0.45\textwidth}{!}
% {
\begin{tabular}{lc}
  \toprule \toprule
    \textbf{Model} & \textbf{Complexity} \\ 
\midrule 
    Transformer \citep{vaswani2017attention} & $O(N^2)$   \\
    Reformer \citep{reformer} & $O(N log N)$   \\
    Longformer \citep{beltagy2020longformer} & $O(N)$  \\
    BigBird \citep{zaheer2020bigbird} & $O(N)$   \\
\midrule
    \mname & $O(N)$ \\
\bottomrule
\end{tabular}
% } % small
\end{center}
\caption{Computational complexity of several related models}
\label{tab:complexity_analysis}
% \vspace{-0.5cm}
\end{table}

==> table/lra_speed_mem.tex <==


\begin{table*}[t]
\begin{center}
\resizebox{0.98\textwidth}{!}
{

\begin{tabular}{l|cccc|cccc}
  \toprule \toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c|}{\textbf{Steps per second ↑}} & \multicolumn{4}{c}{\textbf{Peak Memory Usage (GB) ↓}} \\ 
   & \textbf{1K}  & \textbf{2K} & \textbf{3K} & \textbf{4K} & \textbf{1K}  & \textbf{2K} & \textbf{3K} & \textbf{4K} \\ \hline
    Transformer & 0.71 & 0.73 & 0.77 & 0.67 & 7.66 & 9.76 & 13.11 & 20.20 \\
    \hline
    Local Attention & 0.61(0.9x) & 0.63(0.9x) & 0.73(0.9x) & 0.73(1.1x) & 6.59 & 7.09 & 7.64 & 7.67 \\
    Linformer & 0.81(1.1x) & 0.84(1.2x) & 0.73(0.9x) & 0.77(1.1x) & 6.59 & 7.09 & 7.64 & 7.67 \\
    Reformer & 0.80(1.1x) & 0.78(1.1x) & 0.77(1.0x) & 0.80(1.2x) & 6.59 & 7.67 & 9.68 & 9.74 \\
    Performer & 0.82(1.2x) & 0.82(1.1x) & 0.78(1.0x) & 0.78(1.2x) & 6.59 & 7.09 & 7.64 & 7.67 \\
    Sinkhorn Trans. & 0.82(1.2x) & 0.80(1.1x) & 0.82(1.1x) & 0.79(1.2x) & 6.59 & 7.10 & 7.64 & 7.68 \\
    Synthesizer & 0.76(1.1x) & 0.81(1.1x) & 0.78(1.0x) & 0.57(0.8x) & 7.99 & 11.10 & 16.41 & 27.18 \\
    Longformer & 0.77(1.1x) & 0.77(1.1x) & 0.75(1.0x) & 0.62(0.9x) & 7.67 & 12.99 & 20.27 & 20.29 \\
    Sparse Trans. & 0.77(1.1x) & 0.81(1.1x) & 0.83(1.1x) & 0.65(1.0x) & 7.67 & 9.77 & 13.14 & 20.25 \\
    BigBird & 0.77(1.1x) & 0.76(1.0x) & 0.76(1.0x) & 0.80(1.2x) & 7.09 & 7.64 & 9.68 & 9.68 \\
    \hline
    \mname & 0.80(1.1x) & 0.82(1.1x) & 0.78(1.0x) & 0.78(1.2x) & 7.64 & 9.67 & 13.27 & 12.96 \\
    \mname w/o \textbf{SAR} & 0.79(1.1x) & 0.75(1.0x) & 0.76(1.0x) & 0.81(1.2x) & 7.09 & 7.64 & 9.68 & 9.68 \\
\bottomrule
\end{tabular}

}

\end{center}

\caption{Training speed and peak memory consumption comparison of different models on byte-level text classification with various input lengths (1K, 2K, 3K and 4K) on 8 $\times$ A100 GPU, where Memory Usage is the average across 8 GPU.}
\label{lra_speed_mem}

\end{table*}

==> table/qa_and_cls.tex <==
% \begin{table*}[t]
% \parbox{.49\linewidth}{
% \centering
% \resizebox{0.5\columnwidth}{!}{
% \begin{tabular}{l|ccc}
%   \toprule \toprule
%     \textbf{Models} & \textbf{Arxiv}
%     \tablefootnote{The reported numbers from \citep{zaheer2020bigbird} on Arxiv dataset are not comparable with ours because they did not release the train/test split of the data. So we re-tested RoBERTa and BigBird's open source checkpoint on our Arxiv train/test split. We open source our Arxiv dataset split: https://github.com/anonymous}
%     & \textbf{IMDB}  & \textbf{Hyperpartisan} \\
%     \hline
%                 & F1 & Acc & F1  \\ \hline
%     RoBERTa & 86.86 & 95.00±0.2 & 87.80±0.8  \\
%     % Longformer do not mention the scores are max or average among 5 times repeat, do not consider it here
%     % Longformer  & 95.70 & 94.8  \\
%     % BigBird(paper) & - & 95.20±0.2 & 92.20±1.7  \\
%     % BigBird(reprod)\footnotemark[1] & 87.50 & 94.87±0.1 & 90.63±0.0 \\
%     BigBird & 87.50 & 95.20±0.2 & 92.20±1.7  \\
% \midrule
%     \mname & \textbf{89.05} & \textbf{95.53±0.1} & \textbf{92.81±1.4} \\
% \bottomrule
% \end{tabular}
% }
% \caption{Performance of various models on development set of benchmark natural language understanding tasks. }
% \label{text_cls_experimental_results}
% }
% \hfill
% \parbox{.49\linewidth}{
% \resizebox{0.4\columnwidth}{!}{
% \begin{tabular}{l|ccc}
%   \toprule \toprule
%     \textbf{Models} & \textbf{WikiHop}  & \multicolumn{2}{c}{\textbf{TriviaQA}} \\ 
% \midrule 
%     & Acc & F1 & EM\\
% \midrule 
%     Longformer  & 75.0  & 75.2 & -\\
%     BigBird & 75.9  & 79.5 & - \\
% \midrule
%     \multicolumn{3}{l}{\textbf{Reproduce}} \\
% \midrule 
%     Longformer & 75.2  & 75.0 & 67.0 \\
%     BigBird & 72.3  & 73.4 & 68.6 \\
% \midrule
%     \mname & \textbf{75.8}  & \textbf{76.5} & \textbf{71.8} \\
% \bottomrule
% \end{tabular}
% }
% \caption{Model comparison for WikiHop and TriviaQA.}
% \label{qa_experimental_results}
% }
% \vspace{-0.2cm}
% \end{table*}


\begin{table*}[t]
\parbox{.5\linewidth}{
\centering
\setlength{\extrarowheight}{5pt}
\begin{tabular}{L{5cm}|C{0.8cm}}
  \toprule \toprule
    \textbf{Setting} &  \textbf{BPC}\\[2pt]
\midrule
    RoBERTa  \citep{liu2019roberta}  & 1.85    \\[2pt]
    Longformer \citep{beltagy2020longformer}      & 1.71       \\[2pt]
    BigBird \citep{zaheer2020bigbird}      & 1.68       \\[2pt]
\midrule
    \mname & 1.67     \\[2pt]
\bottomrule
\end{tabular}
\caption{MLM BPC for \mname and other models.}
\label{tab:pretrain_bpc}
}
\hfill
\parbox{.48\linewidth}{
\begin{tabular}{l|ccc}
  \toprule \toprule
    \textbf{Models} & \textbf{WikiHop}  & \multicolumn{2}{c}{\textbf{TriviaQA}} \\ 
\midrule 
    & Acc & F1 & EM\\
\midrule 
    Longformer  & 75.0  & 75.2 & -\\
    BigBird & 75.9  & 79.5 & - \\
\midrule
    \multicolumn{3}{l}{\textbf{Reproduce}} \\
\midrule 
    Longformer & 75.2  & 75.0 & 67.0 \\
    BigBird & 72.3  & 73.4 & 68.6 \\
\midrule
    \mname & \textbf{75.8}  & \textbf{76.5} & \textbf{71.8} \\
\bottomrule
\end{tabular}
\caption{Model comparison for WikiHop and TriviaQA.}
\label{qa_experimental_results}
}
\end{table*}

==> table/qa_and_cls_v2.tex <==


\begin{table*}[t]
\centering
% \small
\begin{tabular}{l|cccccc}
  \toprule \toprule
    \textbf{Models} & \textbf{Arxiv}  & \textbf{IMDB}  & \textbf{Hyp} & \textbf{WikiHop}  & \multicolumn{2}{c}{\textbf{TriviaQA}} \\ \hline
                    & F1              & Acc            & F1           & \textbf{Acc}      & \textbf{F1} & \textbf{EM} \\ \hline
    RoBERTa         & 86.86           & 95.00          & 87.80        & -                 & 74.3        & -           \\
    Longformer      & -               & \textbf{95.70}           & -            & 75.2              & 75.0        & 67.0        \\
    BigBird         & 87.50           & 95.20          & 92.20        & 72.3              & 73.4        & 68.6        \\
\midrule
    \mname          & \textbf{89.05} & 95.53 & \textbf{92.81} &\textbf{75.8}  & \textbf{76.5} & \textbf{71.8} \\
\bottomrule
\end{tabular}
\caption{Performance of various models on development set of benchmark natural language understanding tasks. }
\label{text_cls_and_qa_experimental_results}
\end{table*}

% \tablefootnote{The reported numbers from \citep{zaheer2020bigbird} on Arxiv dataset are not comparable with ours because they did not release the train/test split of the data. So we re-tested RoBERTa and BigBird's open source checkpoint on our Arxiv train/test split. We open source our Arxiv dataset split: https://github.com/anonymous}
